Designing RF-Powered Battery-Less Electronic Shelf Labels With COTS Components

This paper presents a preliminary study exploring the feasibility of designing batteryless electronic shelf labels (ESLs) powered by radio frequency wireless power transfer using commercial off-the-shelf components. The proposed ESL design is validated through a dedicated testbed and involves a detailed analysis of design choices, including energy consumption, energy conversion, and storage solutions. A leaded aluminium electrolytic capacitor is selected as the primary energy storage element, balancing cost and performance while maintaining compactness. Experimental evaluations demonstrate that an ESL can update its display within 4 to 120 minutes, depending on input power and RF frequency, with harvester efficiencies reaching up to 30 %. Challenges such as low harvester efficiency, extended update times, and hardware constraints are identified, highlighting opportunities for future optimizations. This work provides valuable insights into system design considerations for RF-powered ESLs and establishes a foundation for further research in energy-neutral Internet of Things applications.

==> auto_names.tex <==

 
 
 
\makeatletter
\PassOptionsToPackage{dvipsnames,svgnames,table}{xcolor}%
\makeatother


\usepackage{listofitems}
\usepackage{pgffor}
\usepackage{xparse}
\usepackage{ifthen}
\usepackage{tikz}
\usepackage{xspace}
\usetikzlibrary{external}

\makeatletter
\def\myColorList{LimeGreen,BrickRed,Fuchsia,Bittersweet,YellowOrange, YellowGreen, WildStrawberry, Fuchsia, RedViolet, Periwinkle, PineGreen, OrangeRed, RawSienna, Turquoise, Aquamarine, BlueViolet, BurntOrange, DarkOrchid, TealBlue, Violet, RoyalPurple}
\readlist\ColorList\myColorList


\definecolor{defaultColor}{RGB}{112,45,128}
\NewDocumentCommand{\roundLabel}{O{defaultColor} m}{%
\tikzexternaldisable
    \tikz[baseline=(char.base)]{
        \node[rectangle, rounded corners=0.65mm, inner sep=0.65mm, fill=#1, draw=#1, text=white, font=\itshape](char) {#2};
    }%
\tikzexternalenable
}


\NewDocumentCommand{\defineauthors}{ O{true} m }{%
    \ifthenelse{\equal{#1}{true}}{%
        Personal commands for comments are:
        \begin{itemize}
        \foreach \x [count=\xi from 1] in {#2} {   
            \item \textcolor{\ColorList[\xi]}{\textbackslash\unexpanded\expandafter{\x}\{\}}
            }
        \end{itemize}
        \foreach \x [count=\xi from 1] in {#2} { 
            \expandafter\xdef\csname\x\endcsname####1{\noexpand\textcolor{\ColorList[\xi]}{\roundLabel[\ColorList[\xi]]{\unexpanded\expandafter{\x}} ####1}}%
        }
    }{%
        \foreach \x [count=\xi from 1] in {#2} { 
            \expandafter\xdef\csname\x\endcsname####1{\noexpand\textcolor{\ColorList[\xi]}{\roundLabel[\ColorList[\xi]]{\unexpanded\expandafter{\x}} ####1}}%
        }
    }
    \foreach \x [count=\xi from 1] in {#2} {
        \expandafter\xdef\csname at\x\endcsname####1{\noexpand\textcolor{\ColorList[\xi]}{@\x}}%
    }
}

\makeatother


